An Operational Semantic Basis for OpenMP Race Analysis

OpenMP is the de facto standard to exploit the on-node parallelism in new generation supercomputers.Despite its overall ease of use, even expert users are known to create OpenMP programs that harbor concurrency errors, of which one of the most insidious of errors are {\em data races}.OpenMP is also a rapidly evolving standard, which means that future data races may be introduced within unfamiliar contexts.A simple and rigorous operational semantics for OpenMP can help build reliable race checkers and ward off future errors through programmer education and better tooling.This paper's key contribution is a simple operational semantics for OpenMP, with primitive events matching those generated by today's popular OpenMP runtimes and tracing methods such as OMPT.This makes our operational semantics more than a theoretical document for intellectual edification; it can serve as a blueprint for OpenMP event capture and tool building.We back this statement by summarizing the workings of a new data race checker for OpenMP being built based on this semantics.The larger purpose served by our semantics is to serve the needs of the OpenMP community with regard to their contemplated extensions to OpenMP, as well as future tooling efforts.

==> Makefile <==
DEPS = *.tex *.bib

all: root.pdf

root.pdf: root.tex $(DEPS)
	pdflatex root.tex
	bibtex root
	pdflatex root.tex
	pdflatex root.tex

clean:
	rm -f root.pdf *.ps *.dvi *~ \#*\#
	rm -rf figures/*.aux *.aux *.bbl *.blg *.dvi *.log *.rel *.toc *.out *.synctex.gz auto

